LLaRA: Supercharging Robot Learning Data for Vision-Language Policy

Vision Language Models (VLMs) have recently been leveraged to generate robotic actions, forming Vision-Language-Action (VLA) models. However, directly adapting a pretrained VLM for robotic control remains challenging, particularly when constrained by a limited number of robot demonstrations. In this work, we introduce LLaRA: Large Language and Robotics Assistant, a framework that formulates robot action policy as visuo-textual conversations and enables an efficient transfer of a pretrained VLM into a powerful VLA, motivated by the success of visual instruction tuning in Computer Vision. First, we present an automated pipeline to generate conversation-style instruction tuning data for robots from existing behavior cloning datasets, aligning robotic actions with image pixel coordinates. Further, we enhance this dataset in a self-supervised manner by defining six auxiliary tasks, without requiring any additional action annotations. We show that a VLM finetuned with a limited amount of such datasets can produce meaningful action decisions for robotic control. Through experiments across multiple simulated and real-world tasks, we demonstrate that LLaRA achieves state-of-the-art performance while preserving the generalization capabilities of large language models. The code, datasets, and pretrained models are available at https://github.com/LostXine/LLaRA.

==> figs/rulebase_template.tex <==
\begin{figure}[h]
    \centering
    \fbox{\includegraphics[width=1.0\linewidth]{figs/rulebase_template.pdf}}
    \caption{\textbf{Template for the Training Dataset} This figure illustrates the template for the training dataset, which follows the format of the LLaVA training scheme. The spatial reasoning conversation is shown as an example. The human prompting section includes the image and the query, while GPT section provides the expert's answer either from rule-based or LLM, allowing the model to learn from the expert. The terms in curly brackets are placeholders to be replaced with corresponding words. The example shown is part of the rule-based spatial reasoning training dataset.}
    \label{fig:rulebase_template}
\end{figure}

